Fast3R: Towards 3D Reconstruction of 1000+ Images in One Forward Pass

Multi-view 3D reconstruction remains a core challenge in computer vision, particularly in applications requiring accurate and scalable representations across diverse perspectives. Current leading methods such as DUSt3R employ a fundamentally pairwise approach, processing images in pairs and necessitating costly global alignment procedures to reconstruct from multiple views. In this work, we propose Fast 3D Reconstruction (Fast3R), a novel multi-view generalization to DUSt3R that achieves efficient and scalable 3D reconstruction by processing many views in parallel. Fast3R's Transformer-based architecture forwards N images in a single forward pass, bypassing the need for iterative alignment. Through extensive experiments on camera pose estimation and 3D reconstruction, Fast3R demonstrates state-of-the-art performance, with significant improvements in inference speed and reduced error accumulation. These results establish Fast3R as a robust alternative for multi-view applications, offering enhanced scalability without compromising reconstruction accuracy.

==> tab/recon_improvement.tex <==
\begin{table}[h]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{0.3em}
    \begin{tabularx}{0.98\columnwidth}{r >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X}
      \toprule

           \multirow{2}{*}{Method} & \multicolumn{2}{c}{7 scenes} & \multicolumn{2}{c}{NRGBD} & \multicolumn{2}{c}{CO3D} \\
      \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
         & {\tt{Acc}$\downarrow$} & {\tt{Comp}$\downarrow$} & {\tt{Acc}$\downarrow$} & {\tt{Comp}$\downarrow$} & {\tt{Acc}$\downarrow$} & {\tt{Comp}$\downarrow$} \\
      \midrule
      {DUSt3R$^\dagger$} & \bf 1.23 & 0.91 & \bf 2.51 & 1.03 & 1.159 & 0.914 \\
      {Spann3R} & 1.48 & \bf 0.85 & \bf 3.15 & 1.10 & 2.268 & 1.295 \\
      {Fast3R} & 2.84 & 1.37 & 4.39 & 1.28 & 3.913 & 1.411 \\
      \bf {Fast3R (Larger)} & \bf 1.58 &  0.93 &  3.40 & \bf 1.01 & \bf 1.706 & \bf 0.857 \\
      \bottomrule
    \end{tabularx}%
    \vspace{-5pt}

    \caption{Improved 3D reconstruction performance.} 
    \vspace{-10pt}
    \label{tab:quant_recon_scene}
\end{table}


==> tab/reconstruction_full.tex <==

\begin{table*}[h]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{0.3em}
    \begin{tabularx}{\textwidth}{r c c >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >
    {\centering\arraybackslash}X >{\centering\arraybackslash}X >
    {\centering\arraybackslash}X >
    {\centering\arraybackslash}X >{\centering\arraybackslash}X}
      \toprule

           \multirow{3}{*}{Method} & \multicolumn{1}{c}{\multirow{3}{*}{Optim.}} & \multicolumn{1}{c}{\multirow{3}{*}{Onl.}} & \multicolumn{6}{c}{7 scenes~\cite{shotton2013scene}} & \multicolumn{6}{c}{NRGBD~\cite{azinovic2022neural}} & \multirow{3}{*}{FPS} \\

      \cmidrule(lr){4-9} \cmidrule(lr){10-15}
         & & & \multicolumn{2}{c}{\tt{Acc}$\downarrow$} & \multicolumn{2}{c}{\tt{Comp}$\downarrow$} & \multicolumn{2}{c}{\tt{NC}$\uparrow$} & \multicolumn{2}{c}{\tt{Acc}$\downarrow$} & \multicolumn{2}{c}{\tt{Comp}$\downarrow$} & \multicolumn{2}{c}{\tt{NC}$\uparrow$} & \\
      \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15}
         & & & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \\
      \midrule
      \textbf{F-Recon~\cite{xu2023frozenrecon}} &\checkmark &
        & 0.1243 & 0.0762 & 0.0554 & 0.0231 & 0.6189  & 0.6885  & 0.2855  & 0.2059  & 0.1505 & 0.0631  & 0.6547  & 0.7577 & \footnotesize{\textless}0.1 \\
      \textbf{DUSt3R$^\dagger$~\cite{dust3r_cvpr24}} &\checkmark &
        & \bf 0.0286 & \bf 0.0123 & 0.0280 & 0.0091 & \bf 0.6681   & \bf 0.7683  & \bf 0.0544  & \bf 0.0251  & 0.0315  & \bf 0.0103  & \bf 0.8024  & \bf 0.9529  & 0.78 \\
      \textbf{Spann3R~\cite{wang2024spann3r}} & & \checkmark
        & 0.0342 & 0.0148 & \bf 0.0241 & \bf 0.0085 & 0.6635  & 0.7625  & 0.0691  & 0.0315  & \bf 0.0291  & 0.0110  & 0.7775  & 0.9371  & \bf 65.49 \\
      \textbf{Fast3R (ours)} & & \checkmark
        & 0.0502 &	0.0284 & 0.0450	 & 0.0137 &  0.6207 & 0.6895   & 0.0696 & 0.0439 & 0.0322 & 0.0128 & 0.7723 & 0.9319 & \bf 1000+ \\
      \midrule
      \textbf{DUSt3R~\cite{dust3r_cvpr24} (FV)} &\checkmark &
        & \bf 0.0188 & \bf 0.0087 & \bf 0.0234 & \bf 0.0096 & \bf 0.7851   & 0.8985  & \bf 0.0392   &\bf  0.0167 & \bf 0.0342 &\bf  0.0121 & \bf 0.8765   & \bf 0.9757   & 0.48 \\ % 16.5922
    %--------------------------------
      \textbf{DUSt3R$^\dagger$~\cite{dust3r_cvpr24} (FV)} &\checkmark &
        & 0.0279 & 0.0133 & 0.0276 & 0.0108 & 0.7630   & 0.8841  & 0.0591  & 0.0266  & 0.0409  & 0.0136  & 0.8305  & 0.9556  & 1.42 \\ % 5.6088
      \textbf{Spann3R$^\star$~\cite{wang2024spann3r} (FV)} & &
        & 0.0233 &  0.0108 & 0.0246 & 0.0104 & 0.7791  & \bf 0.9003  & 0.0587  & 0.0239 & 0.0390  & 0.0132  & 0.8384  & 0.9616  & 5.83\\ % 1.37
      \textbf{Spann3R~\cite{wang2024spann3r} (FV)} & & \checkmark
        & 0.0239 & 0.0111 & 0.0247 & 0.0103 & 0.7768  & 0.8985  & 0.0611  & 0.0254  & 0.0392  & 0.0135  & 0.8330  & 0.9593  & \bf 72.04\\
     \textbf{Fast3R (ours) (FV)} & & \checkmark
        &  &  &  &  &   &   &   &   &   &   &   &  & \bf \\
      \bottomrule
    \end{tabularx}%
    \vspace{-5pt}

    \caption{\textbf{3D reconstruction results on 7Scenes~\cite{shotton2013scene} and NRGBD~\cite{azinovic2022neural} datasets.} DUSt3R$^\dagger$ indicates using DUSt3R's final weights on $224\times 224$ images, same as our input resolution, to fit within 24GB GPU memory. \sasha{are we useing 224?} \jed{we are using 512 for both training and inference. I also found if we train with 512 and inference with 224, the numbers are much worse than if we inference with 512.}For few-view (FV) reconstruction, we use the 8-frame pairs~\cite{duzceker2021deepvideomvs} as in SimpleRecon~\cite{sayed2022simplerecon}. Note that evaluating DUSt3R at the original resolution may benefit from increased visual overlapping. \jed{Our numbers didn't quite beat other models. I think we have to emphasize we are using an unordered set of images instead of a sequence}} 
    \vspace{-10pt}
    \label{tab:quantitative}
\end{table*}
      
     


\begin{table}[]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{0.3em}
    \begin{tabularx}{\columnwidth}{r c c >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X}
      \toprule

         \multirow{2}{*}{Method} & \multicolumn{1}{c}{\multirow{2}{*}{Opt.}} & \multicolumn{1}{c}{\multirow{2}{*}{Onl.}} & \multicolumn{2}{c}{\tt{Acc}$\downarrow$} & \multicolumn{2}{c}{\tt{Comp}$\downarrow$} & \multicolumn{2}{c}{\tt{NC}$\uparrow$} \\ % \multirow{2}{*}{Speed}
      \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
         & & & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} & \tt{Mean} & \tt{Med.} \\
      \midrule
      
      \textbf{DUSt3R~\cite{dust3r_cvpr24}} &\checkmark &
        & \bf 2.114 &  \bf 1.159 & \bf 2.033 & \bf 0.914 & \bf 0.749 & \bf 0.849\\
      \textbf{DUSt3R$^\dagger$~\cite{dust3r_cvpr24}} &\checkmark &
        & 2.296 &  1.297 & 2.158 & 1.002 & 0.747 & 0.848\\
      \textbf{Spann3R$^\star$} & &
        & 2.902 & 1.273 & 2.120 & 0.937 & 0.732 & 0.836\\
        \textbf{Spann3R} & & \checkmark
        & 4.785 & 2.268 & 2.743 & 1.295 & 0.721 & 0.823\\
        \textbf{Fast3R (Ours)} & & \checkmark
        & 6.194  & 4.017 & 3.146 & 1.411 & 0.640 & 0.707 \\
      \midrule
      \textbf{DUSt3R~\cite{dust3r_cvpr24} (FV)} &\checkmark &
        & \bf 2.128 & \bf 1.241 & \bf 2.464 &  \bf 1.228 & \bf 0.797 & \bf 0.889 \\
      \textbf{DUSt3R$^\dagger$~\cite{dust3r_cvpr24} (FV)} &\checkmark &
        & 2.511 & 1.484 & 2.661 &1.230 & 0.788 &  0.883 \\
      \textbf{Spann3R$^\star$ (FV)} & &
        & 3.055 & 1.600 & 2.878 & 1.345 & 0.781 & 0.878\\
      \textbf{Spann3R (FV)} & & \checkmark
        & 3.375 & 1.782 & 2.870 & 1.338 & 0.777 & 0.875\\
      \textbf{Fast3R (Ours) (FV)} & & \checkmark
        &  &  &  &  &  & \\
      \bottomrule
    \end{tabularx}
    \vspace{-5pt}

    \caption{\textbf{Quantitative results on DTU~\cite{aanaes2016large} dataset.} For few-view (FV) reconstruction, we use pairs provided in MVSNet~\cite{yao2018mvsnet}.} 
    \vspace{-5pt}
    \label{tab:quant_dtu}
\end{table}


